Interpolation for normal bundles of general curves

Given n general points p_1, p_2,..., p_n in P^r, it is natural to ask when there exists a curve C \subset P^r, of degree d and genus g, passing through p_1, p_2,..., p_n. In this paper, we give a complete answer to this question for curves C with nonspecial hyperplane section. This result is a consequence of our main theorem, which states that the normal bundle N_C of a general nonspecial curve of degree d and genus g in P^r (with d >= g + r) has the property of interpolation (i.e. that for a general effective divisor D of any degree on C, either H^0(N_C(-D)) = 0 or H^1(N_C(-D)) = 0), with exactly three exceptions.

==> Interpolation-short.tex <==
\newcommand{\shortversion}{}

\input{Interpolation}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Interpolation-short"
%%% End: 

